Khaos: Dynamically Optimizing Checkpointing for Dependable Distributed Stream Processing

Distributed Stream Processing systems are becoming an increasingly essential part of Big Data processing platforms as users grow ever more reliant on their ability to provide fast access to new results. As such, making timely decisions based on these results is dependent on a system's ability to tolerate failure. Typically, these systems achieve fault tolerance and the ability to recover automatically from partial failures by implementing checkpoint and rollback recovery. However, owing to the statistical probability of partial failures occurring in these distributed environments and the variability of workloads upon which jobs are expected to operate, static configurations will often not meet Quality of Service constraints with low overhead. In this paper we present Khaos, a new approach which utilizes the parallel processing capabilities of virtual cloud automation technologies for the automatic runtime optimization of fault tolerance configurations in Distributed Stream Processing jobs. Our approach employs three subsequent phases which borrows from the principles of Chaos Engineering: establish the steady-state processing conditions, conduct experiments to better understand how the system performs under failure, and use this knowledge to continuously minimize Quality of Service violations. We implemented Khaos prototypically together with Apache Flink and demonstrate its usefulness experimentally.

==> sections/02_background.tex <==

\section{Background}

Relevant background for this paper are distributed stream processing systems, fault tolerance mechanisms in these systems, and the fundamentals of Chaos Engineering.

\subsection{Distributed Stream Processing}

DSP systems are inherently parallel and distributed. Streaming jobs are composed as a dataflow graph where task vertices contain some user-defined logic and streaming edges pass messages between the tasks \cite{SCS17}. They are, in principle, required to operate indefinitely on an unbounded stream of continuous data to produce new results as elements enter the streams. Because streams are unbounded, aggregating events works differently than in batch processing. Here, in order to perform some statistical analysis, aggregates are scoped by \textit{windows}. Windows can either be data-driven, i.e. requiring a certain number of events to progress, or time-driven. Time is an important notion in stream processing which has ramifications for both performance and the consistency of results. Although three separate times can be distinguished in streaming jobs, we only consider \textit{event time} processing. This is where a timestamp is extracted from each event and together with watermarks are used for time-based operations, i.e. the progress of time depends on the data, not on any wall clocks. It has the most impact on performance when compared to the other times, but events are allowed to arrive out-of-order and results to be consistent even in the presence of failures \footnote{Flink: Event Time. URL: https://ci.apache.org/projects/flink/flink-docs-stable/dev/event\_time.html}.

\subsection{Fault Tolerance in DSP Systems}

A distributed system consists of independent processes which communicate asynchronously by passing messages over communication channels. The \textit{global state} of such a system is represented by the instantaneous local state at each process as well as the instantaneous state of the channels, i.e. the messages in transit. Recording the global state is an important paradigm which in the context of fault tolerance allows for the system to be recovered when failures occur. This is achieved by periodically saving, called checkpointing, and then restoring the system to the last saved global state. Recording on-the-fly global states of a distributed system where there are no bounds on message delays, referred to as the snapshot problem, is non-trivial. This is mainly due to both the lack of globally shared memory and a global clock making synchronization between nodes extremely difficult \cite{KRS95} \cite{FLP85}. Thankfully synchronization is not required, preserving causality within a distributed system is enough for recording a consistent global snapshot \cite{FLP85}. This forms the basis of the \textit{Chandy-Lamport algorithm} upon which checkpoint and rollback recovery strategies are based \cite{CL85}. Its goal is to record a set of process and channel states such that, even though the combination of states may never have occurred at the same time, the recorded global state is consistent. Another aspect which needs to be considered is the consistency of results across a pipeline of interacting systems and the effect that events will have on the global state due to failures. For this, certain systems provide fault tolerance guarantees. We only consider the strongest of these, \textit{exactly-once} delivery. It is here where each event is guaranteed to pass through the system once and only once and results are ensured to be correct even in the presence of failures. This, however, introduces overhead that impacts on performance.

\subsection{Chaos Engineering}

Chaos Engineering tests the robustness of a running system through repeated failure injection experiments. Chaos  experiments involve defining a measurable normal state of the system, introducing failures based on realistic failure scenarios, and evaluating the results \cite{BBR+16}. The normal state is defined through metrics that describe the system’s performance under failure-free conditions and reflect the overall health and requirements of the system. After the normal state has been established, realistic failure scenarios are injected. These scenarios can be obtained from previous failures such as an outage or removing a service from a system \cite{BBH+16} or created using expert-level knowledge \cite{AAS+16}. After an experiment has been completed, the results of the experiment are assessed using the metrics that describe the system's normal state \cite{BBR+16}. Regardless of the outcome, Chaos experiments provide valuable information. If the system maintains its normal state, confidence can be gained that the system can tolerate the failure scenario. Otherwise, a weakness that needs to be addressed is identified and an opportunity for improvement is found \cite{AAS+16}.
 
